Know Thyself: Transferable Visual Control Policies Through Robot-Awareness

Training visual control policies from scratch on a new robot typically requires generating large amounts of robot-specific data. How might we leverage data previously collected on another robot to reduce or even completely remove this need for robot-specific data? We propose a "robot-aware control" paradigm that achieves this by exploiting readily available knowledge about the robot. We then instantiate this in a robot-aware model-based RL policy by training modular dynamics models that couple a transferable, robot-aware world dynamics module with a robot-specific, potentially analytical, robot dynamics module. This also enables us to set up visual planning costs that separately consider the robot agent and the world. Our experiments on tabletop manipulation tasks with simulated and real robots demonstrate that these plug-in improvements dramatically boost the transferability of visual model-based RL policies, even permitting zero-shot transfer of visual manipulation skills onto new robots. Project website: https://www.seas.upenn.edu/~hued/rac

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/ablations.tex <==
\begin{wraptable}{R}{0.5\textwidth}
\vspace{-5mm}
\caption{Feature comparison between baselines and the robot-aware dynamics model.}
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule 
Model & \multicolumn{1}{p{1.2cm}}{\centering \footnotesize{Robot} \\ \footnotesize{State}} & \multicolumn{1}{p{1.2cm}}{\centering \footnotesize{Analytical}\\\footnotesize{Dynamics}} & \multicolumn{1}{p{1.2cm}}{\centering \footnotesize{Proxy} \\ \footnotesize{Robot}} & \multicolumn{1}{p{1.2cm}}{\centering \footnotesize{World} \\ \footnotesize{Loss}} \\

\midrule
VF    & -  & -  & -  & -  \\
VF$+$State    & \checkmark   & -  & - & -  \\
CycleGAN $+$ VF$+$State      & \checkmark   & -  & - & -  \\
RA (ours)     & \checkmark  & \checkmark  & \checkmark  & \checkmark  \\
% \midrule
% RA$-$Proxy\&WorldLoss  &  \checkmark  &  \checkmark    & - & - \\
% RA$-$WorldLoss   &  \checkmark  &  \checkmark  &  \checkmark  
%  & - \\
\bottomrule
% \vspace{-8mm}
\end{tabular}
}
\label{tab:baseline_table}
\end{wraptable}

==> tables/architecture.tex <==
\begin{figure}
 \centering
   \includegraphics[width=0.8\textwidth]{figs/wide_architecture.pdf}
 \caption{The visual dynamics architecture is composed of an analytical robot model $P_r$, and the learned  $P_w$ world model. During robot transfer, the target robot's analytical model is used.}
 \label{fig:architecture}
% \vspace{-2mm}
\vspace{-5mm}
\end{figure}


==> tables/concept.tex <==
\begin{figure}[ht]
 \centering
   \includegraphics[width=0.9\textwidth]{figs/wide_teaser.pdf}
 \caption{(Left) As part of our method, robot-aware control (RAC), we propose to factorize visual dynamics into a robot and world model. (Right) The world model is then readily reused with a new robot, permitting plug-and-play transfer.
 %The unseen robot's analytical model is used to predict robot dynamics, permitting easy robot transfer.
 }
 \label{fig:ra-concept}
\vspace{-5mm}
\end{figure}


%\begin{figure}[tp]
%     \centering
%     \begin{subfigure}[t]{0.43\textwidth}
 %        \centering
 %        \includegraphics[width=\textwidth]{figs/train_teaser.pdf}
 %        \caption{Train on WidowX robot}
%          \label{fig:ra-concept-train}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/test_teaser.pdf}
%         \caption{Test on unseen robot}
%         \label{fig:ra-concept-test}
%     \end{subfigure}
%             \caption{(a) As one part of a robot-aware controller, we propose a modular visual dynamics model, that factorizes into a ``world'' dynamics model and analytical robot dynamics model. (b) At test time, the unseen robot's analytical model is used to predict robot dynamics, permitting easy robot transfer. }
%        \label{fig:ra-concept}
%\end{figure}


==> tables/control_results.tex <==
% \begin{wraptable}[11]{R}{0.45\textwidth}
% % \begin{table}
% \vspace{-8mm}
% \caption{Object pushing success rates for zero-shot transfer to an unseen Franka robot.}

% % \jdc{Could we avoid more suffixes here? Perhaps a column for multi-robot training, with check marks for bottom two alone?}

% \centering
% \resizebox{0.45\textwidth}{!}{  
% \begin{tabular}{llcc}
% \toprule
% \thead{Dynamics\\Model} & Cost & \thead{Multi-Robot\\ Training} & Success\\
% \midrule
% VF$+$State & Pixel & -  & 0/30 (0\%)\\
% RA & Pixel  & -  & 0/30 (0\%)\\
% VF$+$State & RA  & - & 6/30 (20\%)\\
% RA & RA   & - & \textbf{22/30} (71\%) \\
% \midrule
% VF$+$State & Pixel & \checkmark & 11/30 (36\%)\\
% RA  & RA   & \checkmark & \textbf{27/30} (90\%) \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:control_eval}
% % \end{table}
% \end{wraptable}

\begin{table}
\caption{Zero-shot control results. All models are trained on a single robot (WidowX200) unless denoted otherwise. Note the CycleGAN baseline is trained on 12k images of the test-time robot.  }
\centering
\resizebox{0.8\textwidth}{!}{  
\begin{tabular}{lcccc}
\toprule
\thead{Dynamics\\Model} & Cost & \thead{Fetch Push\\ (Sim.)} & \thead{Fetch Pick-and-place\\(Sim.)} & \thead{Franka Push\\ (Real)}\\
\midrule
CycleGAN$+$VF$+$State & Pixel & 12/20 (60\%) &  0/20 (0\%) & - \\
VF$+$State            & Pixel      & 0/20 (0\%) &  0/20 (0\%) & 0/30 (0\%) \\
RA                    & Pixel      & 0/20 (0\%) &  0/20 (0\%) & 0/30 (0\%) \\
VF$+$State            & RA      & 12/20 (60\%) &  4/20 (20\%) & 6/30 (20\%) \\
RA                    & RA      & \textbf{18/20} (90\%) & \textbf{8/20} (40\%) & \textbf{22/30} (71\%)\\
\midrule
VF$+$State \small(Multi-robot)   & Pixel  & -  & - & 11/30 (36\%) \\
RA \small(Multi-robot)          & RA      & - & - & \textbf{27/30} (90\%) \\

\bottomrule
\end{tabular}
}
\label{tab:control_eval}
\end{table}


==> tables/control_rollouts.tex <==
%\jd{Why was this itemized list necessary? It looks like V-model, VS-model, RA-model are already introduced, and all we needed to do was say, we were combining them with V-cost and RA-cost. And why ``-model'', but ``-C''?}
%\begin{itemize}[leftmargin=*]
%    \item (\textbf{V-model + V-C}): This is the lower bound VF controller that uses a vanilla model alongside the vanilla cost.
%   \item (\textbf{VS-model + V-C}): This is the baseline VF controller that uses a vanilla-state model alongside the vanilla cost.
%   \item (\textbf{VS-model + RA-C}): This replaces the vanilla cost with the robot-aware cost. We expect this to work better on object-only goal-images than vanilla-cost, as seen in Figure \ref{fig:cost_comparison}.
%    \item (\textbf{RA-model + V-C}): The robot-aware model is paired with the vanilla cost.
 %   \item (\textbf{RA-model + RA-C}): Robot-awareness is incorporated into all parts of the VF pipeline. We expect this to work the best since it improves upon both the prediction and cost of visual foresight.
%\end{itemize}


\begin{figure}[t]
% \setlength{\belowcaptionskip}{-2pt}
  \centering
  \includegraphics[width=0.8\linewidth]{figs/control_rollouts.pdf}

  \caption{Example results from the control experiments (full videos on \href{https://hueds.github.io/rac/}{website}). We show the start, goal, and end states of RA/RA and baseline (VF$+$State/Pixel). The goal image is overlaid on top of the end state for visual reference.} 
  \label{fig:control_rollouts}
%  \vspace{-1cm}
\end{figure}

==> tables/cost_comparison.tex <==
\begin{figure}[t]
  \centering
%   \includegraphics[width=0.3\linewidth]{figs/cost_vis-2.png}
%   \includegraphics[width=0.45\linewidth]{figs/cost_vis_frames_fewer.png}
%  is the cost between the image at the step and the object-only goal image, and on the right are the trajectories and their goal image (separated by red line). Vanilla cost remains high even in the last time-step when the object is in the correct position, while robot-aware cost decreases accordingly by computing cost only in the world region
    \includegraphics[width=0.8\linewidth]{figs/cost_vis.pdf}
  \caption{The behavior of the pixel and RA cost between the current images of a feasible trajectory and the goal image. (Left) The first row shows the trajectory. The next two rows show the heatmaps (pixel-wise norm) between the image and goal for each cost. The heatmaps show high cost values in the robot region, while the RA cost heatmaps correctly have zero cost in the robot region. (Right) The relative pixel cost fails to decrease as the trajectory progresses, while the RA cost correctly decreases.}
  \label{fig:cost_comparison}
\vspace{-6mm}
\end{figure}

==> tables/few_shot_control_results.tex <==
\begin{wraptable}[7]{r}{0.35\textwidth}
% \vspace{-5mm}
\caption{Few-shot transfer to\\ WidowX200 control results.}
\centering
\resizebox{0.4\textwidth}{!}{  
\begin{tabular}{llc}
\toprule
Dynamics Model & Cost & Success\\
\midrule
VF & Pixel      & 4/50 (8\%) \\
RA & RA    & \textbf{40/50} (80\%) \\
\bottomrule
\end{tabular}
}
\label{tab:few_shot_control_eval}
\end{wraptable}

==> tables/human_goal.tex <==
\begin{figure}[ht]
  \begin{center}
    \includegraphics[width=0.4\textwidth]{figs/humangoal.png}
    \caption{Example human goal image.}   \label{fig:human_goal}
  \end{center}
\end{figure} 

==> tables/prediction_results.tex <==
% \begin{table}[h]
% \caption{World dynamics model evaluations, reported as PSNR and SSIM over world regions.}
% \centering
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
%           Model & \multicolumn{2}{c}{\thead{Zero-shot \\ Fetch (Sim)}} & \multicolumn{2}{c}{\thead{Few-shot \\ WidowX200}}  & \multicolumn{2}{c}{\thead{Zero-shot \\ Franka}} \\
% \cmidrule(lr){2-3}
% \cmidrule(lr){4-5}
% \cmidrule(lr){6-7}
% &
% \multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
% \multicolumn{1}{c}{\thead{SSIM $\uparrow$}} &
% \multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
% \multicolumn{1}{c}{\thead{SSIM $\uparrow$}} &
% \multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
% \multicolumn{1}{c}{\thead{SSIM $\uparrow$}}     \\
% \midrule
% VF   & 39.9  & 0.985 & 32.86  & 0.939 & 28.42 & 0.905  \\
% VFS   & -  & -  & 33.05  & 0.941 & 28.31 &  0.894\\
% RA (Ours) & \textbf{41.8}  & \textbf{0.990}  & \textbf{33.26}  & \textbf{0.944}  & 29.63  & \textbf{0.928}\\
% \midrule
% RA-PL   & -  & -  & 33.19  & 0.943 & 29.76 &   0.918\\
% RA-L  & -  & -  & 33.14  & 0.943 & \textbf{29.93} & \textbf{0.928}  \\
% \bottomrule
% \end{tabular}
% \label{tab:sim_0shot_pred_eval}
% \end{table}

\begin{table}[t]
\caption{World prediction evaluations, reported as average world region PSNR and SSIM over 5 timesteps. We compare against conventional models that use image and/or state (VF and VF$+$State).}
\centering
\resizebox{\textwidth}{!}{  
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
          Model & \multicolumn{2}{c}{\thead{Zero-shot \\ Sim. Fetch \\ (Train on WidowX200)}} & \multicolumn{2}{c}{\thead{Few-shot \\ WidowX200 \\ (Train on 3 robots)}}  &
          \multicolumn{2}{c}{\thead{Zero-shot \\ Mod. WidowX200 \\ (Train on 4 robots)}} &
          \multicolumn{2}{c}{\thead{Zero-shot \\ Franka \\ (Train on 4 robots)}} & \multicolumn{2}{c}{\thead{Zero-shot \\ Franka \\ (Train on WidowX200)}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
&
\multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
\multicolumn{1}{c}{\thead{SSIM $\uparrow$}} &
\multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
\multicolumn{1}{c}{\thead{SSIM $\uparrow$}} &
\multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
\multicolumn{1}{c}{\thead{SSIM $\uparrow$}} &
\multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
\multicolumn{1}{c}{\thead{SSIM $\uparrow$}} &
\multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
\multicolumn{1}{c}{\thead{SSIM $\uparrow$}} \\
\midrule
VF   & 39.9  & 0.985 & 32.86  & 0.939 & 30.59 $\pm$ 3.18 & 0.913  $\pm$ 0.04 & 28.31 $\pm$ 3.35 & 0.901 $\pm$ 0.04 & 28.42 $\pm$ 3.43 & 0.905 $\pm$ 0.04  \\
VF$+$State   & -  & -  & 33.05  & 0.941 & 31.03 $\pm$ 3.17 & 0.915 $\pm$ 0.04 &   29.19 $\pm$ 3.02 & 0.901 $\pm$ 0.04 & 28.31 $\pm$ 3.18 &  0.894 $\pm$ 0.05\\
RA (Ours) & \textbf{41.8}  & \textbf{0.990}  & \textbf{33.26}  & \textbf{0.944}  &  \textbf{31.83} $\pm$ 2.88 & \textbf{0.924} $\pm$ 0.03 & \textbf{29.37} $\pm$ 2.93  & \textbf{0.904 $\pm$ 0.04}   & \textbf{29.63 $\pm$ 3.00}  & \textbf{0.928 $\pm$ 0.03} \\
% \midrule
% RA$-$Proxy\&WorldLoss   & -  & -  & 33.19  & 0.943 & 31.54 & 0.923 &   28.84 & 0.895 & 29.76 &   0.918\\
% RA$-$WorldLoss  & -  & -  & 33.14  & 0.943 & 31.67 & 0.923 &  29.13 & 0.903 & \textbf{29.93} & \textbf{0.928}  \\
\bottomrule
\end{tabular}
}
\label{tab:pred_eval}
\end{table}



% \begin{table}[t]
% \caption{World prediction evaluations, reported as average world region PSNR and SSIM over 5 timesteps. We compare against conventional models that use image and/or state (VF and VF$+$State).}
% \centering
% \resizebox{0.5\textwidth}{!}{  
% \begin{tabular}{@{}lcccccccccc@{}}
% \toprule
%           Model  &
%           \multicolumn{2}{c}{\thead{Zero-shot \\ Franka \\ (Train on 4 robots)}} & \multicolumn{2}{c}{\thead{Zero-shot \\ Franka \\ (Train on WidowX200)}} \\
% \cmidrule(lr){2-3}
% \cmidrule(lr){4-5}
% &
% \multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
% \multicolumn{1}{c}{\thead{SSIM $\uparrow$}} &
% \multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
% \multicolumn{1}{c}{\thead{SSIM $\uparrow$}} &\\
% \midrule
% VF    & 28.31  & 0.901  & 28.42  & 0.905  \\
% VF$+$State  &   29.19  & 0.901  & 28.31  &  0.894 \\
% RA (Ours)  & \textbf{29.37}  & \textbf{0.904 }   & \textbf{29.63 }  & \textbf{0.928 } \\
% % \midrule
% % RA$-$Proxy\&WorldLoss   & -  & -  & 33.19  & 0.943 & 31.54 & 0.923 &   28.84 & 0.895 & 29.76 &   0.918\\
% % RA$-$WorldLoss  & -  & -  & 33.14  & 0.943 & 31.67 & 0.923 &  29.13 & 0.903 & \textbf{29.93} & \textbf{0.928}  \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:pred_eval}
% \end{table}



==> tables/prediction_rollouts.tex <==
\begin{figure}[t]
  \centering
    \includegraphics[width=1\linewidth]{figs/prediction_rollouts.pdf}
     \caption{Model outputs of the zero-shot experiments. First row: the RA model is able to predict contact with the green box, while the baseline (VF$+$State) predicts none. Next row: the RA-model models the downward motion of the octopus more accurately. Refer to the \href{https://hueds.github.io/rac/}{website} for videos.}
  \label{fig:prediction_rollouts}
% \vspace{-4mm}
\end{figure}

==> tables/push_objects.tex <==
\begin{figure}[h]
  \centering
    \includegraphics[width=0.5\textwidth]{figs/push_objects.jpg}
  \caption{The objects used in the control experiments. The few-shot WidowX250 transfer experiment used all objects, while the zero-shot Franka experiment used the bear and watermelon. }
  \label{fig:push_objects}
% \vspace{-2mm}
\end{figure}

==> tables/ra_loss_code.tex <==

\begin{algorithm}[ht]
    \caption{\small Pytorch code for the $L_w$ loss.}
    \label{alg:ra-loss}
        \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
        \lstset{
          backgroundcolor=\color{white},
          basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
          columns=fullflexible,
          breaklines=true,
          captionpos=b,
          commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
          keywordstyle=\fontsize{7.2pt}{7.2pt},
          literate={~} {$\sim$}{1},
          escapechar=\&%
        }
\begin{lstlisting}[language=python]
def ra_l1_loss(pred, target, mask):
    """
    pred and target are of images of dim (3, H, W)
    mask is binary segmentation mask of the robot of dim (1, H, W)
    outputs the mean L1 norm of world pixels
    """
    difference = target - pred # (3, H, W)
    # repeat mask across channel axis so we can use it
    # to index the robot region in difference
    robot_region = mask.repeat(3,1,1)
    # ignore the pixel differences in the robot region
    difference[robot_region] = 0
    # compute the l1 norm over the world pixels
    num_world_pixels = (~robot_region).sum()
    l1_per_pixel = diff.abs().sum() / num_world_pixels
    return l1_per_pixel
\end{lstlisting}
\end{algorithm}

==> tables/ra_test_code.tex <==
\begin{algorithm}[ht]
\caption{\textsc{Test}} 
\label{alg:ra-test}
\begin{algorithmic}[1]
  \STATE \textbf{Input:} World model $W$, analytical model $R$, Start image $o(1)$, start mask $M_r(1)$, start state $r(1)$, actions ${a(1), ..., a(T)}$.
  \STATE $\hat O_w = \{\}$
  \STATE $r \gets r(1)$
  \STATE $o_w \gets \mathrm{MaskRobot}(o(1), M_r(1))$ \hfill \COMMENT{// Here we abuse the $o_w$ notation to be the masked image}
  \FOR{$t=1$ {\bfseries to} $T$}
    \STATE $ r' \gets R(r, a)$
    \STATE $\hat{o}' \gets W(o_w, r, r', a(t))$
    \STATE $\hat{o}_w(t+1) \gets (1 - M_{r'}) \circ \hat{o}'$
    \STATE $\hat O_w \gets \hat O_w \cup \hat{o}_w(t+1)$
    \STATE $o_w \gets \mathrm{MaskRobot}(\hat{o}', M_{r'})$
    \STATE $r \gets r'$
  \ENDFOR
  \STATE \RETURN $\hat O_w$
\end{algorithmic}
\end{algorithm}

==> tables/ra_train_code.tex <==
\begin{algorithm}[ht]
\caption{\textsc{Train}} 
\label{alg:ra-train}
\begin{algorithmic}[1]
  \STATE \textbf{Input:} World model $W$, analytical model $R$, image sequence $o(1) \ldots o(T+1)$, mask sequence $M_r(1) \ldots M_r(T+1)$, state sequence $r(1) \ldots r(T+1)$, actions ${a(1), ..., a(T)}$.
  \STATE $\hat O_w \gets \{\}$
  \STATE $O_w  \gets \{(1 - M_{r}(2)) \circ o(2), \ldots ,(1 - M_{r}(T+1)) \circ o(T+1)\}$

  \STATE $o_w \gets \mathrm{MaskRobot}(o(1), M_r(1))$ \hfill \COMMENT{// Here we abuse the $o_w$ notation to be the masked image}
  \FOR{$t=1$ {\bfseries to} $T$}
    \STATE $\hat{o}' \gets W(o_w, r(t), r(t+1), a(t))$
    \STATE $\hat{o}_w(t+1) \gets (1 - M_r(t+1)) \circ \hat{o}'$
    \STATE $\hat O_w \gets \hat O_w \cup \hat{o}_w(t+1)$
    \STATE $o_w \gets \mathrm{MaskRobot}(\hat{o}', M_r(t+1))$
  \ENDFOR
  \STATE Compute world loss (eq. \ref{eq:ra-loss}) between $O_w$ and $\hat O_w$.
  \STATE \RETURN
\end{algorithmic}
\end{algorithm}

==> tables/robot_setup.tex <==
% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.2\textwidth}
%     	\centering
%     	\includegraphics[width=\textwidth]{figs/widowx.jpeg}
%         \caption{\textsc{WidowX200}}\label{fig:widowx_scene}
%     \end{subfigure}
%     \quad
%     \begin{subfigure}[t]{0.2\textwidth}
%     	\centering
%     	\includegraphics[width=\textwidth]{figs/widowx_mod.jpeg}
%         \caption{\textsc{Modified WidowX200}}\label{fig:widowx_mod_scene}
%     \end{subfigure}
%     \quad
%     \begin{subfigure}[t]{0.2\textwidth}
%     	\centering
%     	\includegraphics[width=\textwidth]{figs/franka.jpg}
%         \caption{\textsc{Franka}}\label{fig:franka_scene}
%     \end{subfigure}
%     \caption{
%         Pictures of the WidowX200, modified WidowX200, and Franka robot.  }
%     \label{fig:robots_scene}
% \end{figure}

\begin{wrapfigure}[6]{r}{0.61\textwidth}
\vspace{-11mm}
  \begin{center}
    \includegraphics[width=0.6\textwidth]{figs/robots_row.pdf}
    \caption{WidowX200, Mod.~WidowX200, Franka}   \label{fig:robots_scene}
  \end{center}
\end{wrapfigure} 

==> tables/sim_cost_comparison.tex <==
\begin{figure}[]
  \centering
    \includegraphics[width=0.8\textwidth]{figs/sim_cost_comparison.pdf}
  \caption{ We evaluate the performance of the pixel cost (V-C) and robot-aware cost (RA-C) by running 100 push tasks where the robot must achieve the object-only goal image. Then we visualize for each task, the final pose distance between the object and the object pose in the goal image. The dashed horizontal line indicates the success threshold of 1cm. The robot-aware cost succeeds in most tasks by outputting a sensible cost over the world region, while pixel cost is distorted by the robot.}
  \label{fig:sim_cost_comparison}
% \vspace{-2mm}
\end{figure}





==> tables/sim_modified_widowx_prediction_results.tex <==
\begin{table}[h]
\caption{Zero-shot video prediction results to a modified WidowX200 in simulation. The modified WidowX200 has different color and/or link lengths.}
\centering

\begin{tabular}{@{}lcccccc@{}}
\toprule
          & \multicolumn{2}{c}{\thead{Color Change}} & \multicolumn{2}{c}{\thead{Link Change}} & \multicolumn{2}{c}{\thead{Color and \\ Link Change}}   \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
&
\multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
\multicolumn{1}{c}{\thead{SSIM $\uparrow$}} &
\multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
\multicolumn{1}{c}{\thead{SSIM $\uparrow$}} &
\multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
\multicolumn{1}{c}{\thead{SSIM $\uparrow$}} \\
\midrule
VF   & 37.5  & 0.976  & 42.3  & 0.994 & 40.3 & 0.987 \\
RA (Ours) & \textbf{38.7}  & \textbf{0.985}  & \textbf{45.2}  & \textbf{0.997} & \textbf{40.9} & \textbf{0.991} \\
\bottomrule
\end{tabular}
\label{tab:sim_0shot_pred_eval_sim}
\end{table}

==> tables/sim_push_control_results.tex <==
\begin{wraptable}[11]{R}{0.45\textwidth}
% \begin{table}
\vspace{-8mm}
\caption{Simulated object pushing success rates for zero-shot transfer to an unseen Fetch robot.}

\centering
\resizebox{0.45\textwidth}{!}{  
\begin{tabular}{llc}
\toprule
\thead{Dynamics\\Model} & Cost & Success\\
\midrule
CycleGAN$+$VF$+$State (Few-shot) & Pixel & 12/20 (60\%) \\
VF$+$State & Pixel  & 0/20 (0\%)\\
RA & Pixel   & 0/20 (0\%)\\
VF$+$State & RA   & 12/20 (20\%)\\
RA & RA    & \textbf{18/20} (90\%) \\
\bottomrule
\end{tabular}
}
\label{tab:sim_control_eval}
% \end{table}
\end{wraptable}

==> tables/supp_control_results.tex <==

\begin{table}[h]
\caption{Tabletop pushing success rates for models pre-trained on multiple robots and transferred to the unseen Franka.}
\centering

\begin{tabular}{llc}
\toprule
Model & Cost & \thead{Zero-shot \\Franka }\\
\midrule
VFS & Pixel     &  6/18 (33\%)\\
RA & Pixel     & 0/18 (0\%) \\
VFS & RA     & 9/18 (50\%)\\
RA & RA   & \textbf{16/18} \textbf{(89}\%\textbf{)} \\
\bottomrule
\end{tabular}
\label{tab:supp_control_eval}
% \vspace{-4mm}
\end{table}

==> tables/supp_multiview_cost.tex <==
\begin{table}
\caption{Simulated object pushing using either single-view or multi-view versions of the robot-aware cost.}
\centering
\begin{tabular}{llc}
\toprule
Cost & Success\\
\midrule
RA      & 95/100 (95\%) \\
RA (2 views)    & \textbf{98/100} (98\%) \\
\bottomrule
\end{tabular}

\label{tab:multiview_cost}
\end{table}

==> tables/supp_multiview_pick.tex <==
\begin{table}[ht]
\caption{Adding an additional view improves pick-and-place performance. }
\centering
\begin{tabular}{lccc}
\toprule
\thead{Dynamics\\Model} & Cost & \thead{Fetch \\ Pick-and-Place\\ (1 View)} & \thead{Fetch \\ Pick-and-place\\(2 Views)}\\
\midrule
VF$+$State            & Pixel      & 0/20 (0\%) &  0/20 (0\%)\\
RA                    & Pixel      & 0/20 (0\%) &  0/20 (0\%) \\
VF$+$State            & RA      & 4/20 (20\%) &  8/20 (40\%)  \\
RA                    & RA      & \textbf{8/20} (40\%) & \textbf{14/20} (70\%)\\
\bottomrule
\end{tabular}

\label{tab:supp_mv_control_eval}
\end{table}


==> tables/supp_prediction_results.tex <==
\begin{table}[h]
\caption{World dynamics model evaluations, reported as PSNR and SSIM over world regions.}
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
          Model & \multicolumn{2}{c}{\thead{Zero-shot \\ Mod. WidowX200}}  & \multicolumn{2}{c}{\thead{Zero-shot \\ Franka}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
&
\multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
\multicolumn{1}{c}{\thead{SSIM $\uparrow$}} &
\multicolumn{1}{c}{\thead{PSNR $\uparrow$}} &
\multicolumn{1}{c}{\thead{SSIM $\uparrow$}}   \\
\midrule
VF   &  31.40  & 0.924  & 28.31 & 0.901  \\
VFS   &  31.43 & 0.924 & 29.19 & 0.901  \\
RA-PL   &  31.54 & 0.923 & 28.84 & 0.895   \\
RA-L  & 31.67 & 0.923 & 29.13 & 0.903   \\
RA (Ours) & \textbf{32.12} & \textbf{0.929} & \textbf{29.37}  & \textbf{0.904}  \\
\bottomrule
\end{tabular}
\label{tab:supp_pred_eval}
\end{table}

==> tables/supp_prediction_rollouts.tex <==
\begin{figure}
  \centering
    \includegraphics[width=1\linewidth]{figs/supp_prediction_rollouts.pdf}
     \caption{Qualitative outputs of the zero-shot prediction experiments on models that were pretrained on multiple robots. From left to right, we show the ground truth start, ground truth future, and predictions for the robot-aware model and VFS model. The baseline blurs the bear in the top row, and predicts minimal movement for the octopus in the bottom row.  The proxy robot is visualized in green. Refer to the videos on the website for more visual comparisons.}
  \label{fig:supp_prediction_rollouts}
% \vspace{-4mm}
\end{figure}

==> tables/train_control_results.tex <==
\begin{table}[ht]
\caption{Performance on the training robot.}
\centering
\begin{tabular}{llcc}
\toprule
\thead{Dynamics\\Model} & Cost & \thead{Push\\Success} & \thead{Pick-and-place\\Success}\\
\midrule
VF$+$State & Pixel      & 86/100 (86\%) & 9/20 (45\%) \\
RA & RA    & \textbf{92/100} (92\%) & \textbf{11/20 (55\%)}\\
\bottomrule
\end{tabular}

\label{tab:train_control_eval}
\end{table}
